Secure V2V and V2I Communication in Intelligent Transportation using Cloudlets

Intelligent Transportation System (ITS) is a vision which offers safe, secure and smart travel experience to drivers. This futuristic plan aims to enable vehicles, roadside transportation infrastructures, pedestrian smart-phones and other devices to communicate with one another to provide safety and convenience services. Vehicle to Vehicle (V2V) and Vehicle to Infrastructure (V2I) communication in ITS offers ability to exchange speed, heading angle, position and other environment related conditions amongst vehicles and with surrounding smart infrastructures. In this intelligent setup, vehicles and users communicate and exchange data with random untrusted entities (like vehicles, smart traffic lights or pedestrians) whom they don't know or have met before. The concerns of location privacy and secure communication further deter the adoption of this smarter and safe transportation. In this paper, we present a secure and trusted V2V and V2I communication approach using edge infrastructures where instead of direct peer to peer communication, we introduce trusted cloudlets to authorize, check and verify the authenticity, integrity and ensure anonymity of messages exchanged in the system. Moving vehicles or road side infrastructure are dynamically connected to nearby cloudlets, where security policies can be implemented to sanitize or stop fake messages and prevent rogue vehicles to exchange messages with other vehicles. We also present a formal attribute-based model for V2V and V2I communication, called AB-ITS, along with proof of concept implementation of the proposed solution in AWS IoT platform. This cloudlet supported architecture complements direct V2V or V2I communication, and serves important use cases such as accident or ice-threat warning and other safety applications. Performance metrics of our proposed architecture are also discussed and compared with existing ITS technologies.

==> Figures/mqtt.tex <==
\begin{figure}[t]
\centering
\includegraphics[scale = .65]{Figures/mqtt-v1}
\caption{Edge Cloudlets Supported MQTT Communication}
\label{fig_mqtt}
\end{figure} 

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> Sections/Limitation.tex <==
\section{Discussion and Limitations}\label{sec-limit}

==> Tables/table_conf2.tex <==
\iffalse
\begin{table*}[t]
\centering
\caption{Parameter Information}
\label{tab 6}
\begin{tabular}{|c|c|c|lll}
\cline{1-3}
{\textbf{Admin Role}} &  {\textbf{Prereq. Cond}} & {\textbf{AllowedGroups}} &  &  &  \\ \cline{1-3}
%UniAdmin                                  & NULL                                       & \{UN\}                                       &  &  &  \\ \cline{1-3}
%DeptAdm                                 & \begin{tabular}[c]{@{}c@{}} \{C,Java\} $\subseteq \mathrm{{effective}_{skills}(u) } \;\land $ \\ U $\in$ directUg(u) \end{tabular}                                          & \{CSD\}                                     &  &  &  \\ \cline{1-3}
DeptAdmin                                 & \begin{tabular}[c]{@{}c@{}} \{c, java\} $\subseteq \mathrm{{effective}_{skills}(u) } \;\land $ \\ S $\notin$ effectiveUg(u) \end{tabular}                                          & \{G,CSD\}                                     &  &  &  \\ \cline{1-3}
StaffAdmin                                &  \begin{tabular}[c]{@{}c@{}} \{G,UGR\} $\cap\; \mathrm{effectiveUg(u)= \o \;\land } $ \\ Admin$ \; \in\mathrm{ {effective}_{jobTitle}(u)}$   \end{tabular}                            & \{S\}                                       &  &  &  \\ \cline{1-3}
%DeptAdm                                &  \begin{tabular}[c]{@{}c@{}} U $\in \mathrm{ directUg(u)\;} \land $ \\ graduate $\in \mathrm{ {effective}_{stuType}(u)}$  \end{tabular}                    & \{CSD,G\}                                       &  &  &  \\ \cline{1-3}
%DeptAdm                                &  \begin{tabular}[c]{@{}c@{}} U $\in \mathrm{ directUg(u)\;} \land $ \\ graduate $\in \mathrm{ {effective}_{stuType}(u)}$  \end{tabular}                    & \{CSD,G\}                                       &  &  &  \\ \cline{1-3}
%StudAdm                                 &  \begin{tabular}[c]{@{}c@{}} CSD $\in\mathrm{ effectiveUg(u)\;} \land $\\ 90 $\in \mathrm{ {effective}_{credit}(u)}$   \end{tabular}                                  & \{D,G\}                                     &  &  &  \\ \cline{1-3}
DeptAdmin                                 &  \begin{tabular}[c]{@{}c@{}} U $\in\mathrm{ directUg(u)\;} \land $\\ 3.02 $\in \mathrm{ {roomAcc}(u) \land S  \notin effectiveUg(u)}  $   \end{tabular}                                  & \{UGR,CSD\}                                     &  &  &  \\ \cline{1-3}
\end{tabular}
\end{table*}
\fi
\iffalse
\begin{table}[]
\caption{AWS Setup Parameter Information}
\label{tab-2}
\setlength{\tabcolsep}{5pt} % Default value: 6pt
\renewcommand{\arraystretch}{1.1} % Default value: 1
\begin{tabular}{cc}
\hline
%\multicolumn{1}{|c|}{Average Message Size (Payload)}                                                                  & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}} 153 B (No Alert), \\ 370 B (Alert) \end{tabular}} \\ \hline
\multicolumn{1}{|c|}{Message Queue Size}                                                                              & \multicolumn{1}{c|}{2.5 MB}                                                                     \\ \hline
\multicolumn{1}{|c|}{Number of AWS Greengrass Groups}                                                                 & \multicolumn{1}{c|}{4}                                                                          \\ \hline
\multicolumn{1}{|c|}{Range of Vehicles per groups}                                                                    & \multicolumn{1}{c|}{1 -- 50}                                                                    \\ \hline
\multicolumn{1}{|c|}{\begin{tabular}[c]{@{}c@{}}Published Range of Messages \\ (per second per vehicle)\end{tabular}} & \multicolumn{1}{c|}{1 -- 20}                                                                    \\ \hline
\multicolumn{1}{|c|}{Greengrass Server Configuration}                                                                 & \multicolumn{1}{c|}{8 VCPUs, 4 GB RAM}                                                          \\ \hline
\multicolumn{1}{|c|}{Simulated Vehicles Server Config.}                                                                & \multicolumn{1}{c|}{2 VCPUs, 4 GB RAM}                                                          \\ \hline
\multicolumn{1}{|c|}{Average Network traffic (50 vehicle)}                                                                 & \multicolumn{1}{c|}{ 255 Kbps}                                                          \\ \hline
\multicolumn{1}{|c|}{Network Capacity of Interface}                                                                & \multicolumn{1}{c|}{1.84 Mbps}                                                          \\ \hline
\multicolumn{1}{l}{}                                                                                                  & \multicolumn{1}{l}{}
\end{tabular}
\end{table}
\fi
\iffalse
\begin{table}[]
\caption{Data Traffic Comparison}
\label{tab-3}
\begin{tabular}{|c|c|c|}
\hline
\textbf{Alert Type} & \textbf{\begin{tabular}[c]{@{}c@{}}Allowable latency \\  (ms)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}AB-ITS latency\\ (ms)\end{tabular}} \\ \hline
Accident & $\sim$100 & $\sim$20 \\ \hline
Tire Slip & $\sim$100 & $\sim$20 \\ \hline
Rogue & -- & $\sim$20 \\ \hline
\end{tabular}
\end{table}
\fi

\begin{table*}[]
\caption{Proposed Edge Supported V2V and V2I Data Traffic Comparison}
\label{tab-3}
\centering
\setlength{\tabcolsep}{6pt} % Default value: 6pt
\renewcommand{\arraystretch}{1.2} % Default value: 1
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\textbf{Applications} & \textbf{\begin{tabular}[c]{@{}c@{}}Message Size \\ (bytes)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Allowable latency \\  (ms) in DSRC \cite{Xu:2004:VSM:1023875.1023879} \end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Average AB-ITS\\ latency (ms)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Network \\ Traffic Type\end{tabular}} & \textbf{Priority} \\ \hline
Accident Warning & 319 & $\sim$100 &  & Event & Safety of Life  \\ \hline
Tire Slip Alert & 319 & $\sim$100  &  & Event  & Safety of Life \\ \hline
\begin{tabular}[c]{@{}c@{}}No Alert (Service \\ Announcement)\end{tabular} & 315  & $\sim$500 &  & Periodic & Non-Safety \\ \hline
\begin{tabular}[c]{@{}c@{}}Rogue Vehicle \\ Updates \end{tabular} & \begin{tabular}[c]{@{}c@{}} 40 (Add a vehicle)\\43 (Remove a vehicle) \end{tabular} & NA &  & Periodic  & Non-Safety \\ \hline
\end{tabular}
\end{table*} 

==> Tables/table_model-old.tex <==
\begin{table*}
\centering
%\captionsetup{justification=centering}
\caption{Formal AB-ITS Communication Model Definitions}% \\ (\textsuperscript{**} and \textsuperscript{++} highlights new and modified components respectively w.r.t \heac)}
\label{tab 1}
\renewcommand{\arraystretch}{1.1}
%\resizebox*{!}{\totalheight}
{%
\begin{tabular}{@{}llllll@{}}
\toprule
\multicolumn{6}{l}{\textbf{Basic Sets and  Functions}}\\
\multicolumn{6}{l}{-- V, I, U, TC are finite sets of vehicles, transportation infrastructure devices, users, and trusted cloudlets respectively.}                              \\
\multicolumn{6}{l}{-- S, \vt, OP are finite sets of sources, target vehicles, and operations respectively, where S = I $\cup$ V $\cup$ U and \vt~$\subseteq$ V.}\\
%\multicolumn{6}{l}{-- S = I $\cup$ V $\cup$ U and \vt~$\subseteq$ V}\\
%\multicolumn{6}{l}{-- HS, \ophs (finite set of Hadoop services and operations respectively)}  [blue circles in Figure \ref{fig_model}]                                                    \\
%\multicolumn{6}{l}{-- HS, ES are finite sets of Hadoop services and ecosystem services respectively.}                                                      \\
%\multicolumn{6}{l}{-- OP is a finite sets of operations.}                                                      \\
%\multicolumn{6}{l}{-- A is a finite set of activities which can be performed in system.}                                                      \\
\multicolumn{6}{l}{-- ATT is a finite set of attributes associated with S, TC, and \vt.}                                                      \\
\multicolumn{6}{l}{-- For each attribute att in ATT,  Range(att) is a finite set of atomic values.}
\\
\multicolumn{6}{l}{-- attType: ATT = \{set, atomic\}, defines attributes to be set or atomic valued.}                                                      \\
\multicolumn{6}{l}{\begin{tabular}{@{}l@{}}-- Each attribute att in ATT maps entities in S, TC, and \vt~to attribute values. Formally,\\\;\; att : S $\cup$ TC $\cup$ \vt~ $\cup$ \{system-wide\}$\rightarrow$\; $ \begin{cases} \mathrm{{Range(att)}}~\cup \{\bot\} & \text{if attType(att) = atomic}\\ \mathrm{2^{Range(att)}} & \text{if attType(att) = set} \\ \end{cases}$ \end{tabular}}
\\
\multicolumn{6}{l}{-- POL is a finite set of authorization policies associated with individual S, TC, \vt~and system-wide.}                                                      \\
\multicolumn{6}{l}{\begin{tabular}{@{}l@{}}-- associated\_cloudlets : $ \mathrm{S~\cup } $ \vt~$\rightarrow$ 2$^\mathrm{TC}$,  mapping each source or target vehicles to a set of trusted cloudlets.\\\;\; Equivalently, relations SEA=$(\mathrm{s,tc)$ and\\
 \evt~ $\subseteq$ \vt~$\times$ TC as shown in Figure \ref{fig_model}. \end{tabular}}
%\multicolumn{6}{l}{-- directG : $ \mathrm{CO \rightarrow 2^{G}} $,  mapping each clustered objects to a set of groups, equivalently CGA $ \subseteq \mathrm{CO} \times \mathrm{G}. $}
\\
%\multicolumn{6}{l}{-- member\_vehicles : $ \mathrm{TEC \rightarrow}$ 2$^\mathrm{V_T}$, mapping each edge to its member vehicles, which is calculated from \evt~ $\subseteq$ \vt~$\times$ TEC.}\\
%\multicolumn{6}{l}{-- rootparentG : $ \mathrm{G \rightarrow G} $,  mapping each group to root parent group in hierarchy.}
%\\
%\multicolumn{6}{l}{-- $\mathrm{GH \subseteq G~\times}$ G,  a partial order relation $\succeq_{\textit{g}}$ on G. Equivalently, parentG : $\mathrm{G \rightarrow 2^{G}}$, mapping group to a set of parent groups in hierarchy.}                                                                                                          \\
%\multicolumn{6}{l}{-- parentG : $ \mathrm{G \rightarrow 2^{G}} $,  mapping each group to set of parent groups in hierarchy, equivalently GH $\subseteq$ G $\times$ G.}
%\multicolumn{6}{l}{-- rootGroup : $ \mathrm{G \rightarrow G} $,  mapping each group to root parent group in hierarchy.}
\\
\multicolumn{1}{l}{\textbf{Effective Attributes of Sources and Vehicles (Derived Functions)}}                                                                 \\
\multicolumn{6}{l}{-- For each attribute $\mathrm{att}$ in ATT such that attType(att) = set :}\\
%\multicolumn{6}{l}{\begin{tabular}{@{}l@{}}-- Each attribute att in ATT maps entities in S, CO, O, G to attribute values. Formally,\\\;\; $\mathrm{\effg_{att}}$ : G $\rightarrow$\; $ \begin{cases} \mathrm{{Range(att)}} & \text{if attType(att) = atomic, defined as $\mathrm{\effg_{att}(g_i)}$ = $\mathrm{att(g_i)}$ $\cup$  $\mathrm{\effg_{att}(g_j)}$ such that $\mathrm{{ g_i \; \succeq_{\textit{g}}\; g_j }}$}\\ \mathrm{2^{Range(att)}} & \text{if attType(att) = set} \\ \end{cases}$ \end{tabular}}\\
%\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}-- For each attribute $\mathrm{att}$ in ATT such that attType(att) = set: \\ $ \;\;\;\; \bullet \;\;$ $\mathrm{\effg_{att}}$ : \Gr~$\rightarrow {2^{\range}}$, defined as $\mathrm{\effg_{att}(g_i)}$ = $\mathrm{att(g_i)}$ $\cup$  $ (\mathrm{\bigcup\limits_{ g \; \in\; \{g_j | g_i \; \succeq_{\textit{g}}\; g_j\} } \effg_{att}(g))}$. \end{tabular}} \\
%\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}-- For each attribute $\mathrm{att}$ in ATT such that attType(att) = set : \\ $ \;\;\;\; \bullet \;\;$ $\mathrm{\effg_{att}}$ : \Gr~$\rightarrow {2^{\range}}$, defined as $\mathrm{\effg_{att}(g_i)}$ = $\mathrm{att(g_i)}$ $\cup$  $ (\mathrm{\bigcup\limits_{ g \; \in\; \{g_j | g_i \; \succeq_{\textit{g}}\; g_j\} } \effg_{att}(g))}$. \end{tabular}} \\
%\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}-- For each attribute $\mathrm{att}$ in ATT such that attType(att) = set: \\ $ \;\;\;\; \bullet \;\;$ $\mathrm{\effg_{att}}$ : \Gr~$\rightarrow {2^{\range}}$, defined as $\mathrm{\effg_{att}(g_i)}$ = $\mathrm{att(g_i)}$ $\cup$  $\mathrm{\effg_{att}(g_j)}$ such that $\mathrm{{ g_i \; \succeq_{\textit{g}}\; g_j }}$. \end{tabular}} \\
\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}$ \;\;\;\; \bullet \;\;$ $\mathrm{\effu_{att}}$ : S~$\rightarrow {2^{\range}}$, defined as $\mathrm{\effu_{att}(s)}$ = $\mathrm{att(s)}$ $\cup$  $ \mathrm{att(associated\_cloudlets(s))}$. \end{tabular}} \\
\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}$ \;\;\;\; \bullet \;\;$ $\mathrm{\effo_{att}}$ : \vt~$\rightarrow {2^{\range}}$, defined as $\mathrm{\effo_{att}(v)}$ = $\mathrm{att(v)}$ $\cup$  $\mathrm{ att(associated\_cloudlets(v))}$. \end{tabular}} \\
%\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}-- For each attribute $\mathrm{att}$ in ATT such that attType(att) = atomic: \\ $ \;\;\;\; \bullet \;\;$ $\mathrm{\effg_{att}}$ : \Gr~$\rightarrow {{\range}}$, defined as $\mathrm{\effg_{att}(g_i)}$ = $\mathrm{\effg_{att}(g_j)}$ such that $\mathrm{{ g_i \; \succeq_{\textit{g}}\; g_j }}$. \end{tabular}} \\
\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}-- For each attribute $\mathrm{att}$ in ATT such that attType(att) = atomic : \\ $ \;\;\;\; \bullet \;\;$ $\mathrm{\effg_{att}}$ : S~$\rightarrow {{\range}} \cup \{\bot\}$, \\\;\;\;\;\;\;\;\; defined as $\mathrm{\effg_{att}(s)}$ = $ \begin{cases} \mathrm{att(s)} & \text{if $\forall~\mathrm{tc} \in \mathrm{associated\_cloudlets(s)}.~ \mathrm{att(tc)} = \bot$}\\ \mathrm{\effg_{att}(s)} & \text{if $\exists~\mathrm{associated\_cloudlets(s)}.~ \mathrm{att(associated\_cloudlets(s))} \neq \bot$ then}\\ & \text{select cloudlet $\mathrm{tc}$ with $\mathrm{att(tc)} \neq \bot$ associated most recently.}\end{cases}$ \end{tabular}} \\
\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}$ \;\;\;\; \bullet \;\;$ $\mathrm{\effo_{att}}$ : \vt~$\rightarrow {{\range}} \cup \{\bot\}$,\\\;\;\;\;\;\;\;\; defined as $\mathrm{\effo_{att}(v)}$ = $ \begin{cases} \mathrm{att(v)} & \text{if $\forall~\mathrm{tc} \in \mathrm{associated\_cloudlets(v)}.~ \mathrm{att(tc)} = \bot$}\\ \mathrm{\effg_{att}(v)} & \text{if $\exists~\mathrm{associated\_cloudlets(v)}.~ \mathrm{att(associated\_cloudlets(v))} \neq \bot$ then}\\ & \text{select cloudlet $\mathrm{tc}$ with $\mathrm{att(tc)} \neq \bot$ associated most recently.}\end{cases}$ \end{tabular}} \\

%\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}$ \;\;\;\; \bullet \;\;$ $\mathrm{\effu_{att}}$ : CO~$\rightarrow {{\range}} \cup \{\bot\}$, defined as $\mathrm{\effu_{att}(co)}$ = $ \begin{cases} \mathrm{att(co)} & \text{if $\mathrm{\effg_{att}(directG(co))} = \bot$}\\ \mathrm{\effg_{att}(directG(co))} & \text{otherwise}\\ \end{cases}$ \end{tabular}} \\
%\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}$ \;\;\;\; \bullet \;\;$ $\mathrm{\effo_{att}}$ : O~$\rightarrow {{\range}} \cup \{\bot\}$, defined as $\mathrm{\effo_{att}(o)}$ = $ \begin{cases} \mathrm{att(o)} & \text{if $\mathrm{\effu_{att}(parentCO(o))} = \bot$}\\ \mathrm{\effu_{att}(parentCO(o))} & \text{otherwise}\\ \end{cases}$ \end{tabular}} \\
\midrule

\multicolumn{2}{l}{ \textbf{Authorization Functions (Policies)}}                                                                                                          \\
%\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}-- {Authorization Function:} For each op $\in$ OP, $\mathrm{Auth_{op}(or:S \cup TC, ob:TEI \cup 2^\mathrm{V_T})}$ is a propositional logic formula  returning true or false, \\\;\; which is defined  using the following policy language: \end{tabular}}\\
\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}-- {Authorization Function:} For each op $\in$ OP, $\mathrm{Auth_{op}(s:S, tc:TC)}$ and $\mathrm{Auth_{op}}$(tc : TC, v : \vt) are \\\;\; parameterized propositional logic  formulas returning true or false, defined  using the following policy language: \end{tabular}}\\
\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}$\;\;\;\; \bullet \;\; \mathrm{ \alpha \Coloneqq \alpha \land \alpha \;|\; \alpha \vee \alpha \;|\; (\alpha) \;|\; \neg \alpha \;|\; \exists\; x \in set.\alpha  \;|\; \forall\; x \in set.\alpha \;|\;  set \bigtriangleup set \;|\; } $ $ \mathrm{atomic \in set \;|\;  atomic \notin set }$\end{tabular}} \\

\multicolumn{6}{l}{$ \;\;\;\; \bullet \;\; \bigtriangleup \Coloneqq  \; \subset \;|\; \subseteq \;|\; \nsubseteq \;|\; \cap \;|\; \cup $}\\

\multicolumn{6}{l}{$ \;\;\;\; \bullet \;\;\mathrm{  set \Coloneqq {eff}_{att}(i) \;|\; {att}(i) }$}for $\mathrm{att}$ $\in $ ATT, i $\in$ S $\cup$ \vt~$\cup$ TC $\cup$ \{system-wide\}, attType(att) = set \;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\\
\multicolumn{6}{l}{$ \;\;\;\; \bullet \;\; \mathrm{ atomic \Coloneqq {eff}_{att}(i) \;|\; {att}(i) \;|\; value }$} for $\mathrm{att}$ $\in $ ATT, i $\in$ S $\cup$ \vt~$\cup$ TC $\cup$ \{system-wide\}, attType(att) = atomic \;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\\
\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}-- {Authorization Function Evaluation:} Authorization functions are passed with actual arguments when function call is made, \\\;\; which  are copied to formal parameters stated in the function and attributes for these formal arguments are computed to \\\;\; evaluate decision. \end{tabular}}\\

\midrule
\multicolumn{2}{l}{ \textbf{Authorization Decision}}                                                                                                          \\
%\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}-- A source \s $\in$ S is allowed to perform an operation op $\in$ OP on edge cloudlet \ob $\in$ TC if the effective attributes  of source \s \\\;\; and edge cloudlet \ob satisfy all the required policies stated in $\mathrm{Auth_{op}}$(\s : S, \ob : TC) function.\\\;\; Formally, $\mathrm{Auth_{op}}$(\s : S, \ob : TC) = True, meaning the function returns true when passed with actual \s and \ob parameters.\end{tabular}}\\
\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}-- A source \s $\in$ S is allowed to perform an operation op $\in$ OP on edge cloudlet \ob $\in$ TC if the effective attributes  of \\\;\; source \s  and edge cloudlet \ob satisfy all the required policies stated in $\mathrm{Auth_{op}}$(\s : S, \ob : TC), where \s and \ob \\\;\; are actual parameters. Formally, $\mathrm{Auth_{op}}$(\s : S, \ob : TC) = True.\end{tabular}}\\
%\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}-- A message from source \s $\in$ S is allowed to be sent to a vehicle v $\in$ \vt~if both the source and vehicle are associated with the same \\\;\; trusted edge cloudlet tc $\in$ TC, and all the required policies are included and evaluated to make final decision. Formally, \\\;\; $\mathrm{Authorization_{send}}$(\s : S, v : \vt) $\Rightarrow$ \\\;\; $\exists$ tc. ((s, tc) $\in$ SEA $\land$ (v, tc) $\in$ \evt~$\land$ $\mathrm{Auth_{send}(s:S, tc:TC)}$ $\land$ $\mathrm{Auth_{forward}}$(tc : TC, v : \vt)) $\land$ (System-Wide Policies) = True \end{tabular}}\\
\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}-- A source \s $\in$ S is allowed to send a message to a vehicle \vp $\in$ \vt~if both the source and vehicle are associated with \\\;\; the same trusted  edge cloudlet \ob $\in$ TC, and all the required policies are included and evaluated to make \\\;\; communication authorization decision. \end{tabular}}\\
\midrule
\multicolumn{2}{l}{ \textbf{Authorization Property }}                                                                                                          \\
\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}-- In order to communicate a message between \s $\in$ S and  \vp $\in$ \vt~ requires authorization for individual operations \{send, forward\} \\\;\; $\in$ OP  where  send[\s, \ob] and forward[\ob, \vp] are operation signatures meaning send operation is performed by \s to \ob and \\\;\; forward is  executed by \ob to \vp. The atomic authorization functions evaluated to allow communication between \s and \vp include \\\;\;  $\mathrm{Auth_{send}}$(\s : S, \ob : TC) and $\mathrm{Auth_{forward}}$(\ob : TC, \vp : \vt). Formally, to send a message from \s to \vp needs  \\\;\; $\exists$ \ob $\in$ TC. ($\mathrm{Auth_{send}}$(\s : S, \ob : TC) $\land$ $\mathrm{Auth_{forward}}$(\ob : TC, \vp : \vt)) $\land$ (System-Wide Policies) = True \end{tabular}}
%\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}-- This composite function $\mathrm{Authorization_{send}}$(\s : S, \vp : \vt) for send operation between \s $\in$ S and  \vp $\in$ \vt~ includes authorization for \\\;\; individual operations  \{send, forward\} $\in$ OP between source \s, cloudlet \ob and vehicle \vp, where \s, \ob and \vp are actual parameters. \\\;\; Formally,  $\mathrm{Authorization_{send}}$(\s : S, \vp : \vt) $\Rightarrow$ \\\;\; $\exists$ \ob $\in$ TC. ($\mathrm{Auth_{send}}$(\s : S, \ob : TC) $\land$ $\mathrm{Auth_{forward}}$(\ob : TC, \vp : \vt)) $\land$ (System-Wide Policies) = True \end{tabular}}
\iffalse
\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}-- A message from source s $\in$ S is communicated to a set of vehicles \vt~if both the source and vehicles are associated with same \\\;\; trusted edge infrastructure tc $\in$ TC, and tc is authorized to forward message to member vehicles. System wide defined policies \\\;\; must also be checked and satisfied. Formally, \\
\;\; $\mathrm{Authorization_{send}(s,\mathrm{V_T})}$ $\Rightarrow$   \end{tabular}}
are included and evaluated to make the final decision. \\ These multi-layer policies are evaluated for
\multicolumn{6}{l}{-- \ophs is a finite set of operations on Hadoop services.}                                                      \\
\multicolumn{6}{l}{-- UA, OA are finite sets of user and object attribute functions respectively.}                                                      \\
\multicolumn{6}{l}{-- ESA, HSA are finite sets of ecosystem and Hadoop service attribute functions respectively.}                                                      \\
\multicolumn{6}{l}{-- For each attribute att in UA $\cup$ OA $\cup$ ESA $\cup$ HSA, Range(att) is a finite set of atomic values.}   \\
\multicolumn{6}{l}{-- attType: UA = \{set\}, defines user attributes to be set valued only.}                                                      \\
\multicolumn{6}{l}{-- attType: OA $\cup$ ESA $\cup$ HSA = \{set, atomic\}, defines remaining attributes to be set or atomic valued.}                                                      \\
\multicolumn{6}{l}{-- For each attribute $\mathrm{att_u}$ in UA, $\mathrm{att_u}$ : U $\cup$ G $\rightarrow$\; $\mathrm{2^{Range(att_u)}}$ mapping each user or group to a set of attribute values in $\mathrm{Range(att_u)}$.}                                                      \\
%\multicolumn{6}{l}{-- For each attribute $\mathrm{att_{ob}}$ in OA, $\mathrm{att_{ob}}$ : OB $\rightarrow$\; \Big\{ $\mathrm{2^{Range(att_{ob})}}$ mapping each object to a set of attribute values in $\mathrm{Range(att_{ob})}$.} \\
\multicolumn{6}{l}{\begin{tabular}{@{}l@{}}-- Each attribute $\mathrm{att_{ob}}$ in OA maps objects in OB to attribute values. Formally, $\mathrm{att_{ob}}$ : OB $\rightarrow$\; $ \begin{cases} \mathrm{{Range(att_{ob})}} & \text{if attType(att$\mathrm{_{ob}}$) = atomic}\\ \mathrm{2^{Range(att_{ob})}} & \text{if attType(att$\mathrm{_{ob}}$) = set} \\ \end{cases}$ \end{tabular}}\\
\multicolumn{6}{l}{\begin{tabular}{@{}l@{}}-- Each attribute $\mathrm{att_{es}}$ in ESA maps services in ES to attribute values. Formally, $\mathrm{att_{es}}$ : ES $\rightarrow$\; $ \begin{cases} \mathrm{{Range(att_{es})}} & \text{if attType(att$\mathrm{_{es}}$) = atomic}\\ \mathrm{2^{Range(att_{es})}} & \text{if attType(att$\mathrm{_{es}}$) = set} \\ \end{cases}$ \end{tabular}}\\
\multicolumn{6}{l}{\begin{tabular}{@{}l@{}}-- Each attribute $\mathrm{att_{hs}}$ in HSA maps services in HS to attribute values. Formally, $\mathrm{att_{hs}}$ : HS $\rightarrow$\; $ \begin{cases} \mathrm{{Range(att_{hs})}} & \text{if attType(att$\mathrm{_{hs}}$) = atomic}\\ \mathrm{2^{Range(att_{hs})}} & \text{if attType(att$\mathrm{_{hs}}$) = set} \\ \end{cases}$ \end{tabular}}\\

%\multicolumn{6}{l}{-- For each attribute $\mathrm{att_{es}}$ in ESA, $\mathrm{att_{es}}$ : ES $\rightarrow$\; $\mathrm{2^{Range(att_{es})}}$ mapping each ecosystem service to a set of attribute values in $\mathrm{Range(att_{es})}$.} \\
%\multicolumn{6}{l}{-- For each attribute $\mathrm{att_{hs}}$ in HSA, $\mathrm{att_{hs}}$ : HS $\rightarrow$\; $\mathrm{2^{Range(att_{hs})}}$ mapping each Hadoop service to a set of attribute values in $\mathrm{Range(att_{hs})}$.} \\
%\multicolumn{6}{l}{-- For each att in $ \mathrm{ UA \cup OA }$, Range(att) is a finite set of atomic values}                   \\
%\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}-- For each $ \mathrm{att_u }\; \mathrm{in \; UA, \; att_u } : \mathrm{U \cup UG \rightarrow\;2^{Range(att_u)}}$, mapping each user \\ \;\; and user group to a set of values in $\mathrm{Range(att_u)}$\end{tabular}}\\
%\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}-- For each  $ \mathrm{att_o }\; \mathrm{in \; OA, \; att_o} : \mathrm{O \cup OG   \rightarrow  \;2^{Range(att_o)}}$, mapping each object \\ \;\;  and object group to a set of values in $\mathrm{Range(att_o)}$\end{tabular}}                                                                                                         \\
\multicolumn{6}{l}{-- \dirug~ : $ \mathrm{U \rightarrow 2^{G}} $,  mapping each user to a set of groups, equivalently UGA $ \subseteq \Ur \times \Gr $}                                                                                                          \\
%\rowcolor[HTML]{EFEFEF}
%\multicolumn{6}{l}{-- \textsuperscript{**}\dirur~  : $ \mathrm{U \rightarrow 2^{R}} $,  mapping each user to a set of roles, equivalently URA $ \subseteq \Ur \times \R $}\\
%\rowcolor[HTML]{C0C0C0}
%\rowcolor{lightgray!40}
%\multicolumn{6}{l}{-- \dirgr~ : $ \mathrm{G \rightarrow 2^{R}} $,  mapping each group to a set of roles, equivalently GRA $ \subseteq \Gr \times \R $}\\

\multicolumn{6}{l}{-- $\mathrm{GH \subseteq G \times }$G,  a partial order relation  $\succeq_{\textit{g}}$ on G}                                                                                                          \\
%\multicolumn{6}{l}{-- For each attribute $\mathrm{att_{ob}}$ in OA, $\mathrm{att_{ob}}$ : OB $\rightarrow$\; \Big\{ $\mathrm{2^{Range(att_{ob})}}$ mapping each object to a set of attribute values in $\mathrm{Range(att_{ob})}$.} }\\
%\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}-- For each $ \mathrm{att_u }\; \mathrm{in \; UA, \; att_u } : \mathrm{U \cup UG \rightarrow\;2^{Range(att_u)}}$, mapping each user \\ \;\; and user group to a set of values in $\mathrm{Range(att_u)}$\end{tabular}}\\
\iffalse
\multicolumn{6}{l}{-- $\mathrm{\obtag \subseteq OB \times }$Tag, relation between object and object tags}                                                                                                          \\
\multicolumn{6}{l}{-- $\mathrm{\dataprms = 2^{ES \times (OB~ \cup ~Tag)  \times OP}}$,  set of data and service object permissions}                                                                                                          \\
\multicolumn{6}{l}{-- $\mathrm{\hsprms = 2^{HS \times \ophs}}$,  set of Hadoop services permissions}                                                                                                          \\ \fi
\\
%\multicolumn{6}{l}{-- $\mathrm{OGH \subseteq OG \times }$OG, a partial order relation $\succeq_{og} $ on OG}\\
%[\defaultaddspace]
%\hline
%\rowcolor{lightgray}

%[\defaultaddspace]\\
\multicolumn{1}{l}{\textbf{Effective Attributes of Users (Derived Functions)}}                                                                 \\
\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}-- For each attribute $\mathrm{att_u}$ in UA, \\ $ \;\;\;\; \bullet \;\;$ $\mathrm{\effg_{att_{u}}}$ : \Gr~$\rightarrow {2^{\range}}$, defined as $\mathrm{\effg_{att_{u}}(g_i)}$ = $\mathrm{att_u(g_i)}$ $\cup$  $ (\mathrm{\bigcup\limits_{ g \; \in\; \{g_j | g_i \; \succeq_{\textit{g}}\; g_j\} } \effg_{att_{u}}(g))}$. \end{tabular}} \\
\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}-- For each attribute $\mathrm{att_u}$ in UA, \\ $ \;\;\;\; \bullet \;\;$ $\mathrm{\effu_{att_{u}}}$ : \Ur~$\rightarrow {2^{\range}}$, defined as $\mathrm{\effu_{att_{u}}(u)}$ = $\mathrm{att_u(u)}$ $\cup$  $ (\mathrm{\bigcup\limits_{ g \; \in\; \dirug(u)} \effg_{att_{u}}(g))}$. \end{tabular}} \\


%\multicolumn{1}{l}{\textsuperscript{$\dagger\dagger$}\textbf{Role Permission Assignments}}                                                                 \\
%\multicolumn{1}{l}{\cellcolor{lightgray}\textbf{Role Permission Assignments}}                                                                 \\
%\multicolumn{6}{l}{-- $\mathrm{\pahs \subseteq R \times }$\hsprms,  mapping roles to hadoop service permissions. Alternatively, \hsp}                                                                                                          \\
%\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}-- $ \mathrm{\pahs \subseteq R \times }$\hsprms,  mapping roles to Hadoop service permissions. Alternatively, \;\; \hsp~: (r:\R) $\rightarrow  {2^{\hsprms}}$, defined as \\ \hsp(r) = \{p $|$ (r,p) $\in$ \pahs \} \end{tabular}} \\
%\multicolumn{5}{l}{\cellcolor[HTML]{343434}{Maanak}}\\
%\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}-- $\mathrm{\pads \subseteq R \times }$\dataprms,  mapping roles to object permissions. Alternatively, \\\;\; \dsp~: (r:\R) $\rightarrow  {2^{\dataprms}}$, defined as \dsp(r) = \{p $|$ (r,p) $\in$ \pads \} \end{tabular}}
 %\hline
%\multicolumn{6}{l}{-- $\mathrm{\pads \subseteq R \times }$\dataprms,  mapping roles to data service permissions}                                                                                                          \\
%\multicolumn{6}{l}{-- $\mathrm{\pah \subseteq HS \times HS~ \times}$ \ophs,  mapping hadoop service to hadoop service access}\\

\multicolumn{1}{l}{\textbf{Effective Attributes of Subjects}}                                                                                                          \\
\multicolumn{6}{l}{-- \userSub~: \s $\rightarrow \; $U, mapping each subject to its creator user.}                                                                                                          \\
\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}-- For each attribute $\mathrm{att_u}$ in UA, $ \mathrm{\effu_{att_{u}}} : \s \rightarrow \mathrm{2^{Range(att_u)}}$, mapping of subject s to a set of values for its effective \\\;\; attribute $\mathrm{att_{u}}$. It is required that : $ \mathrm{\effu_{att_{u}}}(\mathrm{s}) \subseteq \mathrm{\effu_{att_{u}}}(\userSub(\mathrm{s}))$. \end{tabular}} \\[\defaultaddspace]\\
%\multicolumn{6}{l}{-- $\mathrm{\pah \subseteq HS~ \times}$ \hsprms,  mapping hadoop service to hadoop service access.}\\
%\multicolumn{6}{l}{ \textsuperscript{$\dagger\dagger$}\textbf{Effective Roles of Users (Derived Functions)} }                                                                                                      \\
%\multicolumn{2}{l}{\cellcolor{lightgray}\textbf{Effective Roles of Users (Derived Functions)} }                                                                                                          \\
%\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}$ \;\;\;\; \bullet \;\; \effgr : \Gr \rightarrow {2^{\R}}$, defined as \;\;\;\;\;\; $ \effgr(\mathrm{g_i}) = \dirgr(\mathrm{g_i}) $ $\cup $ $ (\mathrm{\bigcup\limits_{\forall g \; \in\; \{g_j | g_i \; \succeq_{\textit{g}}\; g_j\} } \effgr(g))}$\end{tabular}} \\
%\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}$ \;\;\;\; \bullet \;\; \effur : \Ur \rightarrow {2^{\R}}$, defined as \\ \;\;\;\;\;\; $ \effur(\mathrm{u}) = \dirur(\mathrm{u}) $ $\cup $ $ (\mathrm{\bigcup\limits_{\forall g \; \in\; \dirug(u)} \effgr(g))}$\end{tabular}} \\[\defaultaddspace]\\
%\multicolumn{2}{l}{\cellcolor{lightgray}\textbf{Effective Roles and Permissions of Subjects}}                                                                                                          \\

\multicolumn{1}{l}{\textbf{ Cross Hadoop Services Trust}}                                                                                                          \\
\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}-- trusted-services : \hs~$\rightarrow {2^{\hs}}$ is a required function to map Hadoop services to a set of trusted Hadoop services. \\ \;\; Equivalently, relation service trust written as $\trianglelefteq$ $\subseteq$ $\hs$ $\times$ $\hs$, where $\mathrm{hs_a}$ $\trianglelefteq$ $\mathrm{hs_b}$ iff $\mathrm{hs_b}$ $\in$ trusted-services($\mathrm{hs_a}$), meaning \\\;\; trustee service $\mathrm{hs_b}$ is trusted by trustor service $\mathrm{hs_a}$ and Hadoop service $\mathrm{hs_b}$ can access service $\mathrm{hs_a}$. \;\;\end{tabular}} \\
%\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}-- $\mathrm{\pah \subseteq HS~ \times}$ \hsprms,  mapping Hadoop service to Hadoop service access.\\ \;\; Alternatively, \hshsp~: (hs:\hs) $\rightarrow  {2^{\hsprms}}$, defined as \\\;\; \hshsp(hs) = \{p $|$ (hs,p) $\in$ \pah \} \end{tabular}} \\
\midrule
\multicolumn{2}{l}{ \textbf{Authorization Functions}}                                                                                                          \\
%\multicolumn{2}{l}{-- {Service Authorization Function:}}                                                                                                          \\
\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}-- {Service Authorization Function:} For each op $\in$ \ophs, $\mathrm{Authorization_{op}(s:S, sr:HS \cup ES)}$ is a propositional logic formula \\\;\; returning true or false, which is defined  using the following policy language: \end{tabular}}\\
\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}$\;\;\;\; \bullet \;\; \mathrm{ \alpha \Coloneqq \alpha \land \alpha \;|\; \alpha \vee \alpha \;|\; (\alpha) \;|\; \neg \alpha \;|\; \exists\; x \in set.\alpha  \;|\; \forall\; x \in set.\alpha \;|\;  set \bigtriangleup set \;|\; } $ $ \mathrm{atomic \in set \;|\;  atomic \notin set }$\end{tabular}} \\

\multicolumn{6}{l}{$ \;\;\;\; \bullet \;\; \bigtriangleup \Coloneqq  \; \subset \;|\; \subseteq \;|\; \nsubseteq \;|\; \cap \;|\; \cup $}\\
\multicolumn{6}{l}{$ \;\;\;\; \bullet \;\;\mathrm{  set \Coloneqq {effective}_{att_{u}}(s) \;|\; {att_{sr}}(sr) }$} for $\mathrm{att_{u}}$ $\in $ UA, sr $\in$ ES $\cup$ HS, attType(att) = set\\
\multicolumn{6}{l}{$ \;\;\;\; \bullet \;\; \mathrm{ atomic \Coloneqq {att_{sr}}(sr) \;|\; value }$} sr $\in$ ES $\cup$ HS, attType(att) = atomic\\
\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}-- {Data or Service Objects Authorization Function:} For each op $\in$ OP on objects ob $\in$ OB belonging to ecosystem service es $\in$ ES, \\\;\; $\mathrm{Authorization_{op}(s:S, es:ES, ob:OB)}$ is a propositional logic formula returning true or false, which is defined  using \\\;\; the policy language stated above with following changes \end{tabular}}\\
\multicolumn{6}{l}{$ \;\;\;\; \bullet \;\;\mathrm{  set \Coloneqq {effective}_{att_{u}}(s) \;|\; {att_{es}}(es)\;|\; {att_{ob}}(ob) }$} for $\mathrm{att_{u}}$ $\in $ UA, attType(att) = set\\
\multicolumn{6}{l}{$ \;\;\;\; \bullet \;\; \mathrm{ atomic \Coloneqq {att_{es}}(es) \;|\; att_{ob}(ob) \;|\; value }$} attType(att) = atomic\\
%\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}A subject $\mathrm{s}$ $\in$ S is allowed to perform an operation op $\in$ OP on an object $\mathrm{ob}$  $\in$ OB in ecosystem service es $\in$  ES  if the effective \\ object permissions of subject s include permissions to object ob or to tag t $\in$ Tag associated with object ob. Formally,\\ (es,ob,op) $\in$ \effdp($\mathrm{s)}$ $\lor$\\ ($\exists$ t) [(ob,t) $\in$  \obtag~$\land$ (es,t,op) $\in$ \effdp($\mathrm{s)}$] \end{tabular}}\\
%\multicolumn{6}{l}{ For each operation \userSub~: \s $\rightarrow \; $U, mapping each subject to its creator user}                                                                                                          \\
%\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}$ \;\;\;\; \bullet \;\; \effur : \s \rightarrow {2^{\R}}$, mapping of subject s to a set of roles. It is required that : \\ \;\;\;\;\;\; $ \effur(\mathrm{s}) \subseteq \effur(\userSub(\mathrm{s})) $ \end{tabular}} \\[\defaultaddspace]
%\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}-- For each $\mathrm{att_u }$ in UA, $ \mathrm{effective_{att_u} :S \rightarrow 2^{Range({att_u})}}$, mapping of subject s \\ \;\; to a set of roles. It is required that : \\ \;\; $ \mathrm {effective_{att_u}(s) \subseteq {effective}_{att_u}(SubUser(s))}$\end{tabular}}\\ [\defaultaddspace]
%\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}$ \;\;\;\; \bullet \;\; \effhp : \s \rightarrow {2^{\hsprms}}$, defined as $ \effhp(\mathrm{s}) =  $  $ \mathrm{\bigcup\limits_{\forall r \; \in\; \effur(s)} \hsp(r)}$\end{tabular}} \\[\defaultaddspace]
%\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}$ \;\;\;\; \bullet \;\; \effdp : \s \rightarrow {2^{\dataprms}}$, defined as $ \effdp(\mathrm{s}) =  $  $ \mathrm{\bigcup\limits_{\forall r \; \in\; \effur(s)} \dsp(r)}$\end{tabular}} \\[\defaultaddspace]
\midrule
\multicolumn{6}{l}{\textbf{Access Operation Decision}}\\
\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}-- A subject $\mathrm{s}$ $\in$ S is allowed to perform an operation op $\in$ \ophs on a service sr $\in$  ES $\cup$ HS  if the effective attributes of subject s and \\\;\; attributes of services satisfy policies stated in $\mathrm{Authorization_{op}(s:S, sr:HS \cup ES)}$. \\\;\; Formally, $\mathrm{Authorization_{op}(s:S, sr:HS \cup ES)}$ = True.
\end{tabular}}  \\
\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}-- A subject $\mathrm{s}$ $\in$ S is allowed to perform an operation op $\in$ OP on an object $\mathrm{ob}$  $\in$ OB in ecosystem service es $\in$  ES  if subject is allowed \\\;\; to access services es and the effective  attributes of subject s, the attributes of object ob and service es satisfy policies in \\\;\; $\mathrm{Authorization_{op}(s:S, es:ES, ob:OB)}$.\\\;\; Formally, $\mathrm{Authorization_{access}(s:S, es:ES)}$ = True $\land$ $\mathrm{Authorization_{op}(s:S, es:ES, ob:OB)}$ = True.
\end{tabular}}      \fi               \\
\bottomrule
%\multicolumn{6}{l}{\textsuperscript{**} and \textsuperscript{$\dagger\dagger$} highlight new and modified components respectively with respect to \heac}\\
\end{tabular}}
\end{table*}


==> Tables/table_model.tex <==
\begin{table*}
\centering
%\captionsetup{justification=centering}
\caption{Formal AB-ITS Communication Model Definitions}% \\ (\textsuperscript{**} and \textsuperscript{++} highlights new and modified components respectively w.r.t \heac)}
\label{tab 1}
\renewcommand{\arraystretch}{1.1}
%\resizebox*{!}{\totalheight}
{%
\begin{tabular}{@{}llllll@{}}
\toprule
\multicolumn{6}{l}{\textbf{Basic Sets and  Functions}}\\
\multicolumn{6}{l}{-- V, I, U, TC are finite sets of vehicles, transportation infrastructure devices, users, and trusted cloudlets respectively.}                              \\
\multicolumn{6}{l}{-- S, \vt, OP are finite sets of sources, target vehicles, and operations respectively, where S = I $\cup$ V $\cup$ U and \vt~$\subseteq$ V.}\\
%\multicolumn{6}{l}{-- S = I $\cup$ V $\cup$ U and \vt~$\subseteq$ V}\\
%\multicolumn{6}{l}{-- HS, \ophs (finite set of Hadoop services and operations respectively)}  [blue circles in Figure \ref{fig_model}]                                                    \\
%\multicolumn{6}{l}{-- HS, ES are finite sets of Hadoop services and ecosystem services respectively.}                                                      \\
%\multicolumn{6}{l}{-- OP is a finite sets of operations.}                                                      \\
%\multicolumn{6}{l}{-- A is a finite set of activities which can be performed in system.}                                                      \\
\multicolumn{6}{l}{-- ATT is a finite set of attributes associated with S, TC, and \vt.}                                                      \\
\multicolumn{6}{l}{-- For each attribute att in ATT,  Range(att) is a finite set of atomic values.}
\\
\multicolumn{6}{l}{-- attType: ATT = \{set, atomic\}, defines attributes to be set or atomic valued.}                                                      \\
\multicolumn{6}{l}{\begin{tabular}{@{}l@{}}-- Each attribute att in ATT maps entities in S, TC, and \vt~to attribute values. Formally,\\\;\; att : S $\cup$ TC $\cup$ \vt~ $\cup$ \{system-wide\}$\rightarrow$\; $ \begin{cases} \mathrm{{Range(att)}}~\cup \{\bot\} & \text{if attType(att) = atomic}\\ \mathrm{2^{Range(att)}} & \text{if attType(att) = set} \\ \end{cases}$ \end{tabular}}
\\
\multicolumn{6}{l}{-- POL is a finite set of authorization policies associated with individual S, TC, \vt~and system-wide.}                                                      \\
\multicolumn{6}{l}{\begin{tabular}{@{}l@{}}-- associated\_cloudlets : $ \mathrm{S~\cup } $ \vt~$\rightarrow$ 2$^\mathrm{TC}$,  mapping each source or target vehicles to a set of trusted cloudlets.\\\;\; Equivalently, relations SEA $\subseteq \mathrm{S} \times \mathrm{TC}$ and \evt~ $\subseteq$ \vt~$\times$ TC as shown in Figure \ref{fig_model}. \end{tabular}}
%\multicolumn{6}{l}{-- directG : $ \mathrm{CO \rightarrow 2^{G}} $,  mapping each clustered objects to a set of groups, equivalently CGA $ \subseteq \mathrm{CO} \times \mathrm{G}. $}
\\
%\multicolumn{6}{l}{-- member\_vehicles : $ \mathrm{TEC \rightarrow}$ 2$^\mathrm{V_T}$, mapping each edge to its member vehicles, which is calculated from \evt~ $\subseteq$ \vt~$\times$ TEC.}\\
%\multicolumn{6}{l}{-- rootparentG : $ \mathrm{G \rightarrow G} $,  mapping each group to root parent group in hierarchy.}
%\\
%\multicolumn{6}{l}{-- $\mathrm{GH \subseteq G~\times}$ G,  a partial order relation $\succeq_{\textit{g}}$ on G. Equivalently, parentG : $\mathrm{G \rightarrow 2^{G}}$, mapping group to a set of parent groups in hierarchy.}                                                                                                          \\
%\multicolumn{6}{l}{-- parentG : $ \mathrm{G \rightarrow 2^{G}} $,  mapping each group to set of parent groups in hierarchy, equivalently GH $\subseteq$ G $\times$ G.}
%\multicolumn{6}{l}{-- rootGroup : $ \mathrm{G \rightarrow G} $,  mapping each group to root parent group in hierarchy.}
\\
\multicolumn{1}{l}{\textbf{Effective Attributes of Sources and Vehicles (Derived Functions)}}                                                                 \\
\multicolumn{6}{l}{-- For each attribute $\mathrm{att}$ in ATT such that attType(att) = set :}\\
%\multicolumn{6}{l}{\begin{tabular}{@{}l@{}}-- Each attribute att in ATT maps entities in S, CO, O, G to attribute values. Formally,\\\;\; $\mathrm{\effg_{att}}$ : G $\rightarrow$\; $ \begin{cases} \mathrm{{Range(att)}} & \text{if attType(att) = atomic, defined as $\mathrm{\effg_{att}(g_i)}$ = $\mathrm{att(g_i)}$ $\cup$  $\mathrm{\effg_{att}(g_j)}$ such that $\mathrm{{ g_i \; \succeq_{\textit{g}}\; g_j }}$}\\ \mathrm{2^{Range(att)}} & \text{if attType(att) = set} \\ \end{cases}$ \end{tabular}}\\
%\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}-- For each attribute $\mathrm{att}$ in ATT such that attType(att) = set: \\ $ \;\;\;\; \bullet \;\;$ $\mathrm{\effg_{att}}$ : \Gr~$\rightarrow {2^{\range}}$, defined as $\mathrm{\effg_{att}(g_i)}$ = $\mathrm{att(g_i)}$ $\cup$  $ (\mathrm{\bigcup\limits_{ g \; \in\; \{g_j | g_i \; \succeq_{\textit{g}}\; g_j\} } \effg_{att}(g))}$. \end{tabular}} \\
%\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}-- For each attribute $\mathrm{att}$ in ATT such that attType(att) = set : \\ $ \;\;\;\; \bullet \;\;$ $\mathrm{\effg_{att}}$ : \Gr~$\rightarrow {2^{\range}}$, defined as $\mathrm{\effg_{att}(g_i)}$ = $\mathrm{att(g_i)}$ $\cup$  $ (\mathrm{\bigcup\limits_{ g \; \in\; \{g_j | g_i \; \succeq_{\textit{g}}\; g_j\} } \effg_{att}(g))}$. \end{tabular}} \\
%\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}-- For each attribute $\mathrm{att}$ in ATT such that attType(att) = set: \\ $ \;\;\;\; \bullet \;\;$ $\mathrm{\effg_{att}}$ : \Gr~$\rightarrow {2^{\range}}$, defined as $\mathrm{\effg_{att}(g_i)}$ = $\mathrm{att(g_i)}$ $\cup$  $\mathrm{\effg_{att}(g_j)}$ such that $\mathrm{{ g_i \; \succeq_{\textit{g}}\; g_j }}$. \end{tabular}} \\
\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}$ \;\;\;\; \bullet \;\;$ $\mathrm{\effu_{att}}$ : S~$\rightarrow {2^{\range}}$, defined as $\mathrm{\effu_{att}(s)}$ = $\mathrm{att(s)}$ $\cup$  $ \mathrm{att(associated\_cloudlets(s))}$. \end{tabular}} \\
\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}$ \;\;\;\; \bullet \;\;$ $\mathrm{\effo_{att}}$ : \vt~$\rightarrow {2^{\range}}$, defined as $\mathrm{\effo_{att}(v)}$ = $\mathrm{att(v)}$ $\cup$  $\mathrm{ att(associated\_cloudlets(v))}$. \end{tabular}} \\
%\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}-- For each attribute $\mathrm{att}$ in ATT such that attType(att) = atomic: \\ $ \;\;\;\; \bullet \;\;$ $\mathrm{\effg_{att}}$ : \Gr~$\rightarrow {{\range}}$, defined as $\mathrm{\effg_{att}(g_i)}$ = $\mathrm{\effg_{att}(g_j)}$ such that $\mathrm{{ g_i \; \succeq_{\textit{g}}\; g_j }}$. \end{tabular}} \\
\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}-- For each attribute $\mathrm{att}$ in ATT such that attType(att) = atomic : \\ $ \;\;\;\; \bullet \;\;$ $\mathrm{\effg_{att}}$ : S~$\rightarrow {{\range}} \cup \{\bot\}$, \\\;\;\;\;\;\;\;\; defined as $\mathrm{\effg_{att}(s)}$ = $ \begin{cases} \mathrm{att(s)} & \text{if $\forall~\mathrm{tc} \in \mathrm{associated\_cloudlets(s)}.~ \mathrm{att(tc)} = \bot$}\\ \mathrm{\effg_{att}(s)} & \text{if $\exists~\mathrm{associated\_cloudlets(s)}.~ \mathrm{att(associated\_cloudlets(s))} \neq \bot$ then}\\ & \text{select cloudlet $\mathrm{tc}$ with $\mathrm{att(tc)} \neq \bot$ associated most recently.}\end{cases}$ \end{tabular}} \\
\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}$ \;\;\;\; \bullet \;\;$ $\mathrm{\effo_{att}}$ : \vt~$\rightarrow {{\range}} \cup \{\bot\}$,\\\;\;\;\;\;\;\;\; defined as $\mathrm{\effo_{att}(v)}$ = $ \begin{cases} \mathrm{att(v)} & \text{if $\forall~\mathrm{tc} \in \mathrm{associated\_cloudlets(v)}.~ \mathrm{att(tc)} = \bot$}\\ \mathrm{\effg_{att}(v)} & \text{if $\exists~\mathrm{associated\_cloudlets(v)}.~ \mathrm{att(associated\_cloudlets(v))} \neq \bot$ then}\\ & \text{select cloudlet $\mathrm{tc}$ with $\mathrm{att(tc)} \neq \bot$ associated most recently.}\end{cases}$ \end{tabular}} \\

%\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}$ \;\;\;\; \bullet \;\;$ $\mathrm{\effu_{att}}$ : CO~$\rightarrow {{\range}} \cup \{\bot\}$, defined as $\mathrm{\effu_{att}(co)}$ = $ \begin{cases} \mathrm{att(co)} & \text{if $\mathrm{\effg_{att}(directG(co))} = \bot$}\\ \mathrm{\effg_{att}(directG(co))} & \text{otherwise}\\ \end{cases}$ \end{tabular}} \\
%\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}$ \;\;\;\; \bullet \;\;$ $\mathrm{\effo_{att}}$ : O~$\rightarrow {{\range}} \cup \{\bot\}$, defined as $\mathrm{\effo_{att}(o)}$ = $ \begin{cases} \mathrm{att(o)} & \text{if $\mathrm{\effu_{att}(parentCO(o))} = \bot$}\\ \mathrm{\effu_{att}(parentCO(o))} & \text{otherwise}\\ \end{cases}$ \end{tabular}} \\
\midrule

\multicolumn{2}{l}{ \textbf{Authorization Functions (Policies)}}                                                                                                          \\
%\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}-- {Authorization Function:} For each op $\in$ OP, $\mathrm{Auth_{op}(or:S \cup TC, ob:TEI \cup 2^\mathrm{V_T})}$ is a propositional logic formula  returning true or false, \\\;\; which is defined  using the following policy language: \end{tabular}}\\
\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}-- {Authorization Function:} For each op $\in$ OP, $\mathrm{Auth_{op}(s:S, tc:TC)}$ and $\mathrm{Auth_{op}}$(tc : TC, v : \vt) are \\\;\; parameterized propositional logic  formulas returning true or false, defined  using the following policy language: \end{tabular}}\\
\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}$\;\;\;\; \bullet \;\; \mathrm{ \alpha \Coloneqq \alpha \land \alpha \;|\; \alpha \vee \alpha \;|\; (\alpha) \;|\; \neg \alpha \;|\; \exists\; x \in set.\alpha  \;|\; \forall\; x \in set.\alpha \;|\;  set \bigtriangleup set \;|\; } $ $ \mathrm{atomic \in set \;|\;  atomic \notin set }$\end{tabular}} \\

\multicolumn{6}{l}{$ \;\;\;\; \bullet \;\; \bigtriangleup \Coloneqq  \; \subset \;|\; \subseteq \;|\; \nsubseteq \;|\; \cap \;|\; \cup $}\\

\multicolumn{6}{l}{$ \;\;\;\; \bullet \;\;\mathrm{  set \Coloneqq {eff}_{att}(i) \;|\; {att}(i) }$}for $\mathrm{att}$ $\in $ ATT, i $\in$ S $\cup$ \vt~$\cup$ TC $\cup$ \{system-wide\}, attType(att) = set \;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\\
\multicolumn{6}{l}{$ \;\;\;\; \bullet \;\; \mathrm{ atomic \Coloneqq {eff}_{att}(i) \;|\; {att}(i) \;|\; value }$} for $\mathrm{att}$ $\in $ ATT, i $\in$ S $\cup$ \vt~$\cup$ TC $\cup$ \{system-wide\}, attType(att) = atomic \;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\\
\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}-- {Authorization Function Evaluation:} Authorization functions are passed with actual arguments when function call is made, \\\;\; which  are copied to formal parameters stated in the function and attributes for these formal arguments are computed to \\\;\; evaluate decision. \end{tabular}}\\

\midrule
\multicolumn{2}{l}{ \textbf{Authorization Decision}}                                                                                                          \\
%\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}-- A source \s $\in$ S is allowed to perform an operation op $\in$ OP on edge cloudlet \ob $\in$ TC if the effective attributes  of source \s \\\;\; and edge cloudlet \ob satisfy all the required policies stated in $\mathrm{Auth_{op}}$(\s : S, \ob : TC) function.\\\;\; Formally, $\mathrm{Auth_{op}}$(\s : S, \ob : TC) = True, meaning the function returns true when passed with actual \s and \ob parameters.\end{tabular}}\\
\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}-- A source \s $\in$ S is allowed to perform an operation op $\in$ OP on edge cloudlet \ob $\in$ TC if the effective attributes  of \\\;\; source \s  and edge cloudlet \ob satisfy all the required policies stated in $\mathrm{Auth_{op}}$(\s : S, \ob : TC), where \s and \ob \\\;\; are actual parameters. Formally, $\mathrm{Auth_{op}}$(\s : S, \ob : TC) = True.\end{tabular}}\\
%\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}-- A message from source \s $\in$ S is allowed to be sent to a vehicle v $\in$ \vt~if both the source and vehicle are associated with the same \\\;\; trusted edge cloudlet tc $\in$ TC, and all the required policies are included and evaluated to make final decision. Formally, \\\;\; $\mathrm{Authorization_{send}}$(\s : S, v : \vt) $\Rightarrow$ \\\;\; $\exists$ tc. ((s, tc) $\in$ SEA $\land$ (v, tc) $\in$ \evt~$\land$ $\mathrm{Auth_{send}(s:S, tc:TC)}$ $\land$ $\mathrm{Auth_{forward}}$(tc : TC, v : \vt)) $\land$ (System-Wide Policies) = True \end{tabular}}\\
\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}-- A source \s $\in$ S is allowed to send a message to a vehicle \vp $\in$ \vt~if both the source and vehicle are associated with \\\;\; the same trusted  edge cloudlet \ob $\in$ TC, and all the required policies are included and evaluated to make \\\;\; communication authorization decision. \end{tabular}}\\
\midrule
\multicolumn{2}{l}{ \textbf{Authorization Property }}                                                                                                          \\
\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}-- In order to communicate a message between \s $\in$ S and  \vp $\in$ \vt~ requires authorization for individual operations \{send, forward\} \\\;\; $\in$ OP  where  send[\s, \ob] and forward[\ob, \vp] are operation signatures meaning send operation is performed by \s to \ob and \\\;\; forward is  executed by \ob to \vp. The atomic authorization functions evaluated to allow communication between \s and \vp include \\\;\;  $\mathrm{Auth_{send}}$(\s : S, \ob : TC) and $\mathrm{Auth_{forward}}$(\ob : TC, \vp : \vt). Formally, to send a message from \s to \vp needs  \\\;\; $\exists$ \ob $\in$ TC. ($\mathrm{Auth_{send}}$(\s : S, \ob : TC) $\land$ $\mathrm{Auth_{forward}}$(\ob : TC, \vp : \vt)) $\land$ (System-Wide Policies) = True \end{tabular}}
%\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}-- This composite function $\mathrm{Authorization_{send}}$(\s : S, \vp : \vt) for send operation between \s $\in$ S and  \vp $\in$ \vt~ includes authorization for \\\;\; individual operations  \{send, forward\} $\in$ OP between source \s, cloudlet \ob and vehicle \vp, where \s, \ob and \vp are actual parameters. \\\;\; Formally,  $\mathrm{Authorization_{send}}$(\s : S, \vp : \vt) $\Rightarrow$ \\\;\; $\exists$ \ob $\in$ TC. ($\mathrm{Auth_{send}}$(\s : S, \ob : TC) $\land$ $\mathrm{Auth_{forward}}$(\ob : TC, \vp : \vt)) $\land$ (System-Wide Policies) = True \end{tabular}}
\iffalse
\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}-- A message from source s $\in$ S is communicated to a set of vehicles \vt~if both the source and vehicles are associated with same \\\;\; trusted edge infrastructure tc $\in$ TC, and tc is authorized to forward message to member vehicles. System wide defined policies \\\;\; must also be checked and satisfied. Formally, \\
\;\; $\mathrm{Authorization_{send}(s,\mathrm{V_T})}$ $\Rightarrow$   \end{tabular}}
are included and evaluated to make the final decision. \\ These multi-layer policies are evaluated for
\multicolumn{6}{l}{-- \ophs is a finite set of operations on Hadoop services.}                                                      \\
\multicolumn{6}{l}{-- UA, OA are finite sets of user and object attribute functions respectively.}                                                      \\
\multicolumn{6}{l}{-- ESA, HSA are finite sets of ecosystem and Hadoop service attribute functions respectively.}                                                      \\
\multicolumn{6}{l}{-- For each attribute att in UA $\cup$ OA $\cup$ ESA $\cup$ HSA, Range(att) is a finite set of atomic values.}   \\
\multicolumn{6}{l}{-- attType: UA = \{set\}, defines user attributes to be set valued only.}                                                      \\
\multicolumn{6}{l}{-- attType: OA $\cup$ ESA $\cup$ HSA = \{set, atomic\}, defines remaining attributes to be set or atomic valued.}                                                      \\
\multicolumn{6}{l}{-- For each attribute $\mathrm{att_u}$ in UA, $\mathrm{att_u}$ : U $\cup$ G $\rightarrow$\; $\mathrm{2^{Range(att_u)}}$ mapping each user or group to a set of attribute values in $\mathrm{Range(att_u)}$.}                                                      \\
%\multicolumn{6}{l}{-- For each attribute $\mathrm{att_{ob}}$ in OA, $\mathrm{att_{ob}}$ : OB $\rightarrow$\; \Big\{ $\mathrm{2^{Range(att_{ob})}}$ mapping each object to a set of attribute values in $\mathrm{Range(att_{ob})}$.} \\
\multicolumn{6}{l}{\begin{tabular}{@{}l@{}}-- Each attribute $\mathrm{att_{ob}}$ in OA maps objects in OB to attribute values. Formally, $\mathrm{att_{ob}}$ : OB $\rightarrow$\; $ \begin{cases} \mathrm{{Range(att_{ob})}} & \text{if attType(att$\mathrm{_{ob}}$) = atomic}\\ \mathrm{2^{Range(att_{ob})}} & \text{if attType(att$\mathrm{_{ob}}$) = set} \\ \end{cases}$ \end{tabular}}\\
\multicolumn{6}{l}{\begin{tabular}{@{}l@{}}-- Each attribute $\mathrm{att_{es}}$ in ESA maps services in ES to attribute values. Formally, $\mathrm{att_{es}}$ : ES $\rightarrow$\; $ \begin{cases} \mathrm{{Range(att_{es})}} & \text{if attType(att$\mathrm{_{es}}$) = atomic}\\ \mathrm{2^{Range(att_{es})}} & \text{if attType(att$\mathrm{_{es}}$) = set} \\ \end{cases}$ \end{tabular}}\\
\multicolumn{6}{l}{\begin{tabular}{@{}l@{}}-- Each attribute $\mathrm{att_{hs}}$ in HSA maps services in HS to attribute values. Formally, $\mathrm{att_{hs}}$ : HS $\rightarrow$\; $ \begin{cases} \mathrm{{Range(att_{hs})}} & \text{if attType(att$\mathrm{_{hs}}$) = atomic}\\ \mathrm{2^{Range(att_{hs})}} & \text{if attType(att$\mathrm{_{hs}}$) = set} \\ \end{cases}$ \end{tabular}}\\

%\multicolumn{6}{l}{-- For each attribute $\mathrm{att_{es}}$ in ESA, $\mathrm{att_{es}}$ : ES $\rightarrow$\; $\mathrm{2^{Range(att_{es})}}$ mapping each ecosystem service to a set of attribute values in $\mathrm{Range(att_{es})}$.} \\
%\multicolumn{6}{l}{-- For each attribute $\mathrm{att_{hs}}$ in HSA, $\mathrm{att_{hs}}$ : HS $\rightarrow$\; $\mathrm{2^{Range(att_{hs})}}$ mapping each Hadoop service to a set of attribute values in $\mathrm{Range(att_{hs})}$.} \\
%\multicolumn{6}{l}{-- For each att in $ \mathrm{ UA \cup OA }$, Range(att) is a finite set of atomic values}                   \\
%\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}-- For each $ \mathrm{att_u }\; \mathrm{in \; UA, \; att_u } : \mathrm{U \cup UG \rightarrow\;2^{Range(att_u)}}$, mapping each user \\ \;\; and user group to a set of values in $\mathrm{Range(att_u)}$\end{tabular}}\\
%\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}-- For each  $ \mathrm{att_o }\; \mathrm{in \; OA, \; att_o} : \mathrm{O \cup OG   \rightarrow  \;2^{Range(att_o)}}$, mapping each object \\ \;\;  and object group to a set of values in $\mathrm{Range(att_o)}$\end{tabular}}                                                                                                         \\
\multicolumn{6}{l}{-- \dirug~ : $ \mathrm{U \rightarrow 2^{G}} $,  mapping each user to a set of groups, equivalently UGA $ \subseteq \Ur \times \Gr $}                                                                                                          \\
%\rowcolor[HTML]{EFEFEF}
%\multicolumn{6}{l}{-- \textsuperscript{**}\dirur~  : $ \mathrm{U \rightarrow 2^{R}} $,  mapping each user to a set of roles, equivalently URA $ \subseteq \Ur \times \R $}\\
%\rowcolor[HTML]{C0C0C0}
%\rowcolor{lightgray!40}
%\multicolumn{6}{l}{-- \dirgr~ : $ \mathrm{G \rightarrow 2^{R}} $,  mapping each group to a set of roles, equivalently GRA $ \subseteq \Gr \times \R $}\\

\multicolumn{6}{l}{-- $\mathrm{GH \subseteq G \times }$G,  a partial order relation  $\succeq_{\textit{g}}$ on G}                                                                                                          \\
%\multicolumn{6}{l}{-- For each attribute $\mathrm{att_{ob}}$ in OA, $\mathrm{att_{ob}}$ : OB $\rightarrow$\; \Big\{ $\mathrm{2^{Range(att_{ob})}}$ mapping each object to a set of attribute values in $\mathrm{Range(att_{ob})}$.} }\\
%\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}-- For each $ \mathrm{att_u }\; \mathrm{in \; UA, \; att_u } : \mathrm{U \cup UG \rightarrow\;2^{Range(att_u)}}$, mapping each user \\ \;\; and user group to a set of values in $\mathrm{Range(att_u)}$\end{tabular}}\\
\iffalse
\multicolumn{6}{l}{-- $\mathrm{\obtag \subseteq OB \times }$Tag, relation between object and object tags}                                                                                                          \\
\multicolumn{6}{l}{-- $\mathrm{\dataprms = 2^{ES \times (OB~ \cup ~Tag)  \times OP}}$,  set of data and service object permissions}                                                                                                          \\
\multicolumn{6}{l}{-- $\mathrm{\hsprms = 2^{HS \times \ophs}}$,  set of Hadoop services permissions}                                                                                                          \\ \fi
\\
%\multicolumn{6}{l}{-- $\mathrm{OGH \subseteq OG \times }$OG, a partial order relation $\succeq_{og} $ on OG}\\
%[\defaultaddspace]
%\hline
%\rowcolor{lightgray}

%[\defaultaddspace]\\
\multicolumn{1}{l}{\textbf{Effective Attributes of Users (Derived Functions)}}                                                                 \\
\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}-- For each attribute $\mathrm{att_u}$ in UA, \\ $ \;\;\;\; \bullet \;\;$ $\mathrm{\effg_{att_{u}}}$ : \Gr~$\rightarrow {2^{\range}}$, defined as $\mathrm{\effg_{att_{u}}(g_i)}$ = $\mathrm{att_u(g_i)}$ $\cup$  $ (\mathrm{\bigcup\limits_{ g \; \in\; \{g_j | g_i \; \succeq_{\textit{g}}\; g_j\} } \effg_{att_{u}}(g))}$. \end{tabular}} \\
\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}-- For each attribute $\mathrm{att_u}$ in UA, \\ $ \;\;\;\; \bullet \;\;$ $\mathrm{\effu_{att_{u}}}$ : \Ur~$\rightarrow {2^{\range}}$, defined as $\mathrm{\effu_{att_{u}}(u)}$ = $\mathrm{att_u(u)}$ $\cup$  $ (\mathrm{\bigcup\limits_{ g \; \in\; \dirug(u)} \effg_{att_{u}}(g))}$. \end{tabular}} \\


%\multicolumn{1}{l}{\textsuperscript{$\dagger\dagger$}\textbf{Role Permission Assignments}}                                                                 \\
%\multicolumn{1}{l}{\cellcolor{lightgray}\textbf{Role Permission Assignments}}                                                                 \\
%\multicolumn{6}{l}{-- $\mathrm{\pahs \subseteq R \times }$\hsprms,  mapping roles to hadoop service permissions. Alternatively, \hsp}                                                                                                          \\
%\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}-- $ \mathrm{\pahs \subseteq R \times }$\hsprms,  mapping roles to Hadoop service permissions. Alternatively, \;\; \hsp~: (r:\R) $\rightarrow  {2^{\hsprms}}$, defined as \\ \hsp(r) = \{p $|$ (r,p) $\in$ \pahs \} \end{tabular}} \\
%\multicolumn{5}{l}{\cellcolor[HTML]{343434}{Maanak}}\\
%\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}-- $\mathrm{\pads \subseteq R \times }$\dataprms,  mapping roles to object permissions. Alternatively, \\\;\; \dsp~: (r:\R) $\rightarrow  {2^{\dataprms}}$, defined as \dsp(r) = \{p $|$ (r,p) $\in$ \pads \} \end{tabular}}
 %\hline
%\multicolumn{6}{l}{-- $\mathrm{\pads \subseteq R \times }$\dataprms,  mapping roles to data service permissions}                                                                                                          \\
%\multicolumn{6}{l}{-- $\mathrm{\pah \subseteq HS \times HS~ \times}$ \ophs,  mapping hadoop service to hadoop service access}\\

\multicolumn{1}{l}{\textbf{Effective Attributes of Subjects}}                                                                                                          \\
\multicolumn{6}{l}{-- \userSub~: \s $\rightarrow \; $U, mapping each subject to its creator user.}                                                                                                          \\
\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}-- For each attribute $\mathrm{att_u}$ in UA, $ \mathrm{\effu_{att_{u}}} : \s \rightarrow \mathrm{2^{Range(att_u)}}$, mapping of subject s to a set of values for its effective \\\;\; attribute $\mathrm{att_{u}}$. It is required that : $ \mathrm{\effu_{att_{u}}}(\mathrm{s}) \subseteq \mathrm{\effu_{att_{u}}}(\userSub(\mathrm{s}))$. \end{tabular}} \\[\defaultaddspace]\\
%\multicolumn{6}{l}{-- $\mathrm{\pah \subseteq HS~ \times}$ \hsprms,  mapping hadoop service to hadoop service access.}\\
%\multicolumn{6}{l}{ \textsuperscript{$\dagger\dagger$}\textbf{Effective Roles of Users (Derived Functions)} }                                                                                                      \\
%\multicolumn{2}{l}{\cellcolor{lightgray}\textbf{Effective Roles of Users (Derived Functions)} }                                                                                                          \\
%\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}$ \;\;\;\; \bullet \;\; \effgr : \Gr \rightarrow {2^{\R}}$, defined as \;\;\;\;\;\; $ \effgr(\mathrm{g_i}) = \dirgr(\mathrm{g_i}) $ $\cup $ $ (\mathrm{\bigcup\limits_{\forall g \; \in\; \{g_j | g_i \; \succeq_{\textit{g}}\; g_j\} } \effgr(g))}$\end{tabular}} \\
%\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}$ \;\;\;\; \bullet \;\; \effur : \Ur \rightarrow {2^{\R}}$, defined as \\ \;\;\;\;\;\; $ \effur(\mathrm{u}) = \dirur(\mathrm{u}) $ $\cup $ $ (\mathrm{\bigcup\limits_{\forall g \; \in\; \dirug(u)} \effgr(g))}$\end{tabular}} \\[\defaultaddspace]\\
%\multicolumn{2}{l}{\cellcolor{lightgray}\textbf{Effective Roles and Permissions of Subjects}}                                                                                                          \\

\multicolumn{1}{l}{\textbf{ Cross Hadoop Services Trust}}                                                                                                          \\
\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}-- trusted-services : \hs~$\rightarrow {2^{\hs}}$ is a required function to map Hadoop services to a set of trusted Hadoop services. \\ \;\; Equivalently, relation service trust written as $\trianglelefteq$ $\subseteq$ $\hs$ $\times$ $\hs$, where $\mathrm{hs_a}$ $\trianglelefteq$ $\mathrm{hs_b}$ iff $\mathrm{hs_b}$ $\in$ trusted-services($\mathrm{hs_a}$), meaning \\\;\; trustee service $\mathrm{hs_b}$ is trusted by trustor service $\mathrm{hs_a}$ and Hadoop service $\mathrm{hs_b}$ can access service $\mathrm{hs_a}$. \;\;\end{tabular}} \\
%\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}-- $\mathrm{\pah \subseteq HS~ \times}$ \hsprms,  mapping Hadoop service to Hadoop service access.\\ \;\; Alternatively, \hshsp~: (hs:\hs) $\rightarrow  {2^{\hsprms}}$, defined as \\\;\; \hshsp(hs) = \{p $|$ (hs,p) $\in$ \pah \} \end{tabular}} \\
\midrule
\multicolumn{2}{l}{ \textbf{Authorization Functions}}                                                                                                          \\
%\multicolumn{2}{l}{-- {Service Authorization Function:}}                                                                                                          \\
\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}-- {Service Authorization Function:} For each op $\in$ \ophs, $\mathrm{Authorization_{op}(s:S, sr:HS \cup ES)}$ is a propositional logic formula \\\;\; returning true or false, which is defined  using the following policy language: \end{tabular}}\\
\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}$\;\;\;\; \bullet \;\; \mathrm{ \alpha \Coloneqq \alpha \land \alpha \;|\; \alpha \vee \alpha \;|\; (\alpha) \;|\; \neg \alpha \;|\; \exists\; x \in set.\alpha  \;|\; \forall\; x \in set.\alpha \;|\;  set \bigtriangleup set \;|\; } $ $ \mathrm{atomic \in set \;|\;  atomic \notin set }$\end{tabular}} \\

\multicolumn{6}{l}{$ \;\;\;\; \bullet \;\; \bigtriangleup \Coloneqq  \; \subset \;|\; \subseteq \;|\; \nsubseteq \;|\; \cap \;|\; \cup $}\\
\multicolumn{6}{l}{$ \;\;\;\; \bullet \;\;\mathrm{  set \Coloneqq {effective}_{att_{u}}(s) \;|\; {att_{sr}}(sr) }$} for $\mathrm{att_{u}}$ $\in $ UA, sr $\in$ ES $\cup$ HS, attType(att) = set\\
\multicolumn{6}{l}{$ \;\;\;\; \bullet \;\; \mathrm{ atomic \Coloneqq {att_{sr}}(sr) \;|\; value }$} sr $\in$ ES $\cup$ HS, attType(att) = atomic\\
\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}-- {Data or Service Objects Authorization Function:} For each op $\in$ OP on objects ob $\in$ OB belonging to ecosystem service es $\in$ ES, \\\;\; $\mathrm{Authorization_{op}(s:S, es:ES, ob:OB)}$ is a propositional logic formula returning true or false, which is defined  using \\\;\; the policy language stated above with following changes \end{tabular}}\\
\multicolumn{6}{l}{$ \;\;\;\; \bullet \;\;\mathrm{  set \Coloneqq {effective}_{att_{u}}(s) \;|\; {att_{es}}(es)\;|\; {att_{ob}}(ob) }$} for $\mathrm{att_{u}}$ $\in $ UA, attType(att) = set\\
\multicolumn{6}{l}{$ \;\;\;\; \bullet \;\; \mathrm{ atomic \Coloneqq {att_{es}}(es) \;|\; att_{ob}(ob) \;|\; value }$} attType(att) = atomic\\
%\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}A subject $\mathrm{s}$ $\in$ S is allowed to perform an operation op $\in$ OP on an object $\mathrm{ob}$  $\in$ OB in ecosystem service es $\in$  ES  if the effective \\ object permissions of subject s include permissions to object ob or to tag t $\in$ Tag associated with object ob. Formally,\\ (es,ob,op) $\in$ \effdp($\mathrm{s)}$ $\lor$\\ ($\exists$ t) [(ob,t) $\in$  \obtag~$\land$ (es,t,op) $\in$ \effdp($\mathrm{s)}$] \end{tabular}}\\
%\multicolumn{6}{l}{ For each operation \userSub~: \s $\rightarrow \; $U, mapping each subject to its creator user}                                                                                                          \\
%\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}$ \;\;\;\; \bullet \;\; \effur : \s \rightarrow {2^{\R}}$, mapping of subject s to a set of roles. It is required that : \\ \;\;\;\;\;\; $ \effur(\mathrm{s}) \subseteq \effur(\userSub(\mathrm{s})) $ \end{tabular}} \\[\defaultaddspace]
%\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}-- For each $\mathrm{att_u }$ in UA, $ \mathrm{effective_{att_u} :S \rightarrow 2^{Range({att_u})}}$, mapping of subject s \\ \;\; to a set of roles. It is required that : \\ \;\; $ \mathrm {effective_{att_u}(s) \subseteq {effective}_{att_u}(SubUser(s))}$\end{tabular}}\\ [\defaultaddspace]
%\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}$ \;\;\;\; \bullet \;\; \effhp : \s \rightarrow {2^{\hsprms}}$, defined as $ \effhp(\mathrm{s}) =  $  $ \mathrm{\bigcup\limits_{\forall r \; \in\; \effur(s)} \hsp(r)}$\end{tabular}} \\[\defaultaddspace]
%\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}$ \;\;\;\; \bullet \;\; \effdp : \s \rightarrow {2^{\dataprms}}$, defined as $ \effdp(\mathrm{s}) =  $  $ \mathrm{\bigcup\limits_{\forall r \; \in\; \effur(s)} \dsp(r)}$\end{tabular}} \\[\defaultaddspace]
\midrule
\multicolumn{6}{l}{\textbf{Access Operation Decision}}\\
\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}-- A subject $\mathrm{s}$ $\in$ S is allowed to perform an operation op $\in$ \ophs on a service sr $\in$  ES $\cup$ HS  if the effective attributes of subject s and \\\;\; attributes of services satisfy policies stated in $\mathrm{Authorization_{op}(s:S, sr:HS \cup ES)}$. \\\;\; Formally, $\mathrm{Authorization_{op}(s:S, sr:HS \cup ES)}$ = True.
\end{tabular}}  \\
\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}-- A subject $\mathrm{s}$ $\in$ S is allowed to perform an operation op $\in$ OP on an object $\mathrm{ob}$  $\in$ OB in ecosystem service es $\in$  ES  if subject is allowed \\\;\; to access services es and the effective  attributes of subject s, the attributes of object ob and service es satisfy policies in \\\;\; $\mathrm{Authorization_{op}(s:S, es:ES, ob:OB)}$.\\\;\; Formally, $\mathrm{Authorization_{access}(s:S, es:ES)}$ = True $\land$ $\mathrm{Authorization_{op}(s:S, es:ES, ob:OB)}$ = True.
\end{tabular}}      \fi               \\
\bottomrule
%\multicolumn{6}{l}{\textsuperscript{**} and \textsuperscript{$\dagger\dagger$} highlight new and modified components respectively with respect to \heac}\\
\end{tabular}}
\end{table*}

